NIFF: Alleviating Forgetting in Generalized Few-Shot Object Detection via Neural Instance Feature Forging

Privacy and memory are two recurring themes in a broad conversation about the societal impact of AI. These concerns arise from the need for huge amounts of data to train deep neural networks. A promise of Generalized Few-shot Object Detection (G-FSOD), a learning paradigm in AI, is to alleviate the need for collecting abundant training samples of novel classes we wish to detect by leveraging prior knowledge from old classes (i.e., base classes). G-FSOD strives to learn these novel classes while alleviating catastrophic forgetting of the base classes. However, existing approaches assume that the base images are accessible, an assumption that does not hold when sharing and storing data is problematic. In this work, we propose the first data-free knowledge distillation (DFKD) approach for G-FSOD that leverages the statistics of the region of interest (RoI) features from the base model to forge instance-level features without accessing the base images. Our contribution is three-fold: (1) we design a standalone lightweight generator with (2) class-wise heads (3) to generate and replay diverse instance-level base features to the RoI head while finetuning on the novel data. This stands in contrast to standard DFKD approaches in image classification, which invert the entire network to generate base images. Moreover, we make careful design choices in the novel finetuning pipeline to regularize the model. We show that our approach can dramatically reduce the base memory requirements, all while setting a new standard for G-FSOD on the challenging MS-COCO and PASCAL-VOC benchmarks.

==> tables/main_reg_baselines.tex <==
\begin{table*}
\small
\setlength{\tabcolsep}{10pt}
    \centering
    \resizebox{0.9\textwidth}{!}{\begin{tabular}{c | c c c | c c c | c c c}
      \Xhline{1pt}
      \multirow{2}{*}{\textbf{Methods} / \textbf{Shots}} & \multicolumn{3}{c |}{\textbf{5 shot}}  &
      \multicolumn{3}{c |}{\textbf{10 shot}}  &
      \multicolumn{3}{c}{\textbf{30 shot}}\\
      & AP &  bAP & nAP & AP &  bAP & nAP & AP & bAP & nAP \\ \Xhline{1pt}
      \Xhline{1pt}
      DeFRCN~\cite{defrcn} & 23.7 & 26.3 & \second{15.6} & 18.2 & 18.5 & 17.4 & 16.3 & 16.3 & 21.4\\
      DeFRCN + DA & 22.6 & 25.0 & 15.3 & 26.4& 29.2 & 17.9  & 24.2 & 25.0 & 21.8 \\
      \Xhline{1pt}
      DeFRCN w/MAS   & 31.0 & 36.8 & 13.5 & 32.1 & 37.0 & 17.1  & 32.6 & 36.6 & 20.4\\
      DeFRCN w/mMAS  & 30.0 & 35.4 & 13.5 & 30.8 & 35.3 & 17.3  & 32.7 & 36.6 & 20.8\\
      DeFRCN w/LOD   & 29.0 & 34.1 & 13.4 & 29.7  & 34.3 & 16.0 & 29.8 & 33.2 & 19.7 \\
      DeFRCN w/EWC   & 31.5 & 37.6 & 13.4 & 32.4 & 37.5 & 16.8  & 33.0 & 37.3 & 20.1\\
      DeFRCN w/mEWC  & 29.6 & 35.1 & 13.1 & 30.3 & 34.9 & 16.4  & 30.9 & 34.5 & 20.1\\
      DeFRCN w/mEWC + DA  & 30.0 & 35.4 & 13.7 & 31.1 & 36.3 & 15.4 & 31.2 & 34.7 & 20.5  \\
      \Xhline{1pt}
      DeFRCN w/RealFeats.             & 25.2 & 28.9 & 13.8 & 25.8 & 28.9 & 16.6 & 25.5 & 27.3 & 20.1\\
      DeFRCN w/RealFeats. + CFA       & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0\\
      DeFRCN w/RealFeats. + KD        & 26.9 & 31.1 & 14.2 & 27.0 & 30.2 & 17.4 & 27.4 & 29.7 & 20.6\\
      DeFRCN w/RealFeats. + KD + CFA  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0\\
      \Xhline{1pt}
      \rowcolor[HTML]{EFEFEF}
      NIFF-DeFRCN & \best{31.3} & \second{36.3} & \best{15.7} & \best{32.2} & \second{36.6} & \best{19.1} & \best{33.1} & \second{37.2} & 21.0 \\
      %\midrule[1.5pt]
      \Xhline{1pt}
    \end{tabular}}
    \vspace{-0.5em}
    \caption{G-FSOD results of further regularized-based model configurations on MS-COCO for $5,10,30$-shot settings. All experiments are conducted without utilizing base data. DA denotes data augmentations. The {\color{red}best} and {\color{blue}second-best} results for each evaluation protocol are color coded. \vspace{-1.5em}}
    \label{tab:reg_baselines_coco}
\end{table*}
